Sentence Encoders on STILTs: Supplementary Training on Intermediate Labeled-data Tasks

Pretraining sentence encoders with language modeling and related unsupervised tasks has recently been shown to be very effective for language understanding tasks. By supplementing language model-style pretraining with further training on data-rich supervised tasks, such as natural language inference, we obtain additional performance improvements on the GLUE benchmark. Applying supplementary training on BERT (Devlin et al., 2018), we attain a GLUE score of 81.8---the state of the art (as of 02/24/2019) and a 1.4 point improvement over BERT. We also observe reduced variance across random restarts in this setting. Our approach yields similar improvements when applied to ELMo (Peters et al., 2018a) and Radford et al. (2018)'s model. In addition, the benefits of supplementary training are particularly pronounced in data-constrained regimes, as we show in experiments with artificially limited training data.

==> old_tables.tex <==

\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lr@{$\pm$}rr@{$\pm$}rr@{$\pm$}rr@{$\pm$}rr@{$\pm$}rr@{$\pm$}rr@{$\pm$}rr@{$\pm$}r}
\toprule
\textbf{} & 
\multicolumn{2}{c}{\textbf{CoLA}} & \multicolumn{2}{c}{\textbf{SST}} & \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{STS}} & \multicolumn{2}{c}{\textbf{MNLI}} & \multicolumn{2}{c}{\textbf{QNLI}} & \multicolumn{2}{c}{\textbf{RTE}}\\
\textbf{Training Set Size}&
\multicolumn{2}{c}{\textit{8.5k}} & \multicolumn{2}{c}{\textit{67k}} & \multicolumn{2}{c}{\textit{3.7k}} & \multicolumn{2}{c}{\textit{364k}} & \multicolumn{2}{c}{\textit{7k}} & \multicolumn{2}{c}{\textit{393k}} & \multicolumn{2}{c}{\textit{108k}} & \multicolumn{2}{c}{\textit{2.5k}}\\
\midrule
\midrule
\multicolumn{17}{c}{All Training Examples for Target Tasks} \\
\midrule
\textbf{BERT} & 43.3 & 25.8 & \multicolumn{2}{c}{-} & 82.6 & 6.9 & \multicolumn{2}{c}{-} & 88.4 & 4.9 & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & 57.1 & 7.6 \\
 & \multicolumn{2}{c}{(62.1)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.6)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.2)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(70.0)} \\
\textbf{BERT$\rightarrow$QQP} & 34.3 & 25.9 & \multicolumn{2}{c}{-} & 85.1 & 4.8 & \multicolumn{2}{c}{-} & 90.2 & 0.3 & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & 61.8 & 9.5 \\
 & \multicolumn{2}{c}{(56.8)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.4)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.8)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(74.7)} \\
\textbf{BERT$\rightarrow$MNLI} & 49.9 & 17.8 & \multicolumn{2}{c}{-} & 89.7 & 0.5 & \multicolumn{2}{c}{-} & 90.4 & 0.4 & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & 79.2 & 6.4 \\
 & \multicolumn{2}{c}{(59.8)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.9)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.9)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(83.4)} \\
\textbf{BERT$\rightarrow$SNLI} & 40.0 & 23.9 & \multicolumn{2}{c}{-} & 84.3 & 6.4 & \multicolumn{2}{c}{-} & 90.2 & 0.4 & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & 76.0 & 6.6 \\
 & \multicolumn{2}{c}{(57.0)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.1)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(90.7)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(80.1)} \\
\textbf{BERT$\rightarrow$Real/Fake} & 33.4 & 20.5 & \multicolumn{2}{c}{-} & 76.2 & 3.4 & \multicolumn{2}{c}{-} & 32.3 & 42.3 & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & 52.9 & 3.1 \\
 & \multicolumn{2}{c}{(52.4)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(85.7)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(88.6)} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{(59.6)} \\
\midrule
\midrule
\multicolumn{17}{c}{At Most 5k Training Examples for Target Tasks} \\
\midrule
\textbf{BERT} & 35.7 & 27.2 & 81.4 & 18.1 & 80.7 & 6.6 & 67.0 & 21.1 & 82.9 & 21.1 & 58.9 & 20.9 & 76.6 & 11.5 & 57.4 & 8.2  \\
 & \multicolumn{2}{c}{(60.6)} & \multicolumn{2}{c}{(93.5)} & \multicolumn{2}{c}{(89.1)} & \multicolumn{2}{c}{(80.9)} & \multicolumn{2}{c}{(90.0)} & \multicolumn{2}{c}{(77.1)} & \multicolumn{2}{c}{(82.8)} & \multicolumn{2}{c}{(74.0)}  \\
\textbf{BERT$\rightarrow$QQP} & 39.2 & 23.3 & 90.6 & 0.9 & 84.0 & 5.6 & 88.5 & 0.2 & 76.9 & 32.4 & 68.3 & 15.1 & 73.8 & 12.3 & 64.5 & 9.1  \\
 & \multicolumn{2}{c}{(55.3)} & \multicolumn{2}{c}{(92.0)} & \multicolumn{2}{c}{(89.7)} & \multicolumn{2}{c}{(88.9)} & \multicolumn{2}{c}{(90.6)} & \multicolumn{2}{c}{(75.9)} & \multicolumn{2}{c}{(81.6)} & \multicolumn{2}{c}{(76.5)}  \\
\textbf{BERT$\rightarrow$MNLI} & 48.5 & 16.7 & 89.4 & 9.1 & 89.3 & 1.1 & 73.0 & 17.9 & 85.3 & 22.1 & 85.0 & 0.3 & 79.5 & 10.1 & 79.0 & 6.3  \\
 & \multicolumn{2}{c}{(59.6)} & \multicolumn{2}{c}{(92.4)} & \multicolumn{2}{c}{(91.0)} & \multicolumn{2}{c}{(80.9)} & \multicolumn{2}{c}{(90.9)} & \multicolumn{2}{c}{(85.6)} & \multicolumn{2}{c}{(83.9)} & \multicolumn{2}{c}{(83.4)}  \\
\textbf{BERT$\rightarrow$SNLI} & 37.3 & 22.4 & 89.8 & 1.0 & 86.1 & 5.0 & 65.3 & 22.6 & 85.6 & 20.8 & 77.7 & 10.8 & 77.1 & 11.7 & 72.9 & 11.2  \\
 & \multicolumn{2}{c}{(56.6)} & \multicolumn{2}{c}{(91.5)} & \multicolumn{2}{c}{(89.9)} & \multicolumn{2}{c}{(80.4)} & \multicolumn{2}{c}{(90.7)} & \multicolumn{2}{c}{(80.6)} & \multicolumn{2}{c}{(82.7)} & \multicolumn{2}{c}{(80.5)}  \\
\textbf{BERT$\rightarrow$Real/Fake} & 29.5 & 22.9 & 63.8 & 17.0 & 76.2 & 3.3 & 40.4 & 18.0 & 39.1 & 40.6 & 36.4 & 7.1 & 53.4 & 8.3 & 52.1 & 2.0  \\
 & \multicolumn{2}{c}{(53.6)} & \multicolumn{2}{c}{(88.9)} & \multicolumn{2}{c}{(85.1)} & \multicolumn{2}{c}{(78.9)} & \multicolumn{2}{c}{(88.4)} & \multicolumn{2}{c}{(59.1)} & \multicolumn{2}{c}{(74.1)} & \multicolumn{2}{c}{(54.9)}  \\
\midrule
\midrule
\multicolumn{17}{c}{At Most 1k Training Examples for Target Tasks} \\
\midrule
\textbf{BERT} & 39.1 & 17.5 & 77.5 & 17.9 & 79.8 & 3.7 & 65.0 & 17.4 & 80.8 & 20.2 & 45.9 & 13.7 & 68.6 & 9.9 & 57.3 & 7.2  \\
 & \multicolumn{2}{c}{(54.0)} & \multicolumn{2}{c}{(91.1)} & \multicolumn{2}{c}{(86.1)} & \multicolumn{2}{c}{(76.8)} & \multicolumn{2}{c}{(88.0)} & \multicolumn{2}{c}{(69.7)} & \multicolumn{2}{c}{(77.0)} & \multicolumn{2}{c}{(69.0)}  \\
\textbf{BERT$\rightarrow$QQP} & 31.1 & 16.6 & 82.9 & 11.4 & 81.0 & 2.1 & 87.8 & 0.4 & 83.1 & 13.8 & 54.4 & 13.1 & 73.8 & 2.2 & 59.9 & 8.3  \\
 & \multicolumn{2}{c}{(47.5)} & \multicolumn{2}{c}{(89.7)} & \multicolumn{2}{c}{(84.5)} & \multicolumn{2}{c}{(88.6)} & \multicolumn{2}{c}{(88.5)} & \multicolumn{2}{c}{(67.5)} & \multicolumn{2}{c}{(76.4)} & \multicolumn{2}{c}{(71.5)}  \\
\textbf{BERT$\rightarrow$MNLI} & 31.2 & 16.5 & 86.5 & 8.6 & 84.5 & 1.6 & 71.8 & 13.8 & 87.1 & 0.7 & 84.2 & 0.4 & 76.4 & 6.3 & 79.2 & 1.5  \\
 & \multicolumn{2}{c}{(44.0)} & \multicolumn{2}{c}{(90.5)} & \multicolumn{2}{c}{(87.8)} & \multicolumn{2}{c}{(77.3)} & \multicolumn{2}{c}{(88.7)} & \multicolumn{2}{c}{(84.9)} & \multicolumn{2}{c}{(79.0)} & \multicolumn{2}{c}{(82.7)}  \\
\textbf{BERT$\rightarrow$SNLI} & 26.0 & 20.2 & 79.6 & 14.8 & 82.5 & 3.2 & 69.1 & 16.2 & 86.5 & 1.1 & 73.7 & 10.9 & 71.8 & 9.6 & 72.7 & 7.1  \\
 & \multicolumn{2}{c}{(47.6)} & \multicolumn{2}{c}{(89.3)} & \multicolumn{2}{c}{(85.3)} & \multicolumn{2}{c}{(77.4)} & \multicolumn{2}{c}{(88.0)} & \multicolumn{2}{c}{(78.6)} & \multicolumn{2}{c}{(77.6)} & \multicolumn{2}{c}{(79.1)}  \\
\textbf{BERT$\rightarrow$Real/Fake} & 16.3 & 18.0 & 52.6 & 5.2 & 75.2 & 1.9 & 43.8 & 16.9 & 9.9 & 22.7 & 32.8 & 1.2 & 51.1 & 4.4 & 52.1 & 3.7  \\
 & \multicolumn{2}{c}{(43.9)} & \multicolumn{2}{c}{(72.5)} & \multicolumn{2}{c}{(81.8)} & \multicolumn{2}{c}{(71.2)} & \multicolumn{2}{c}{(82.8)} & \multicolumn{2}{c}{(35.3)} & \multicolumn{2}{c}{(69.7)} & \multicolumn{2}{c}{(61.7)}  \\
\bottomrule
\end{tabular}
\caption{Statistics of GLUE results based on 20 random restarts for each experiment for BERT. The numbers reported follow the format: Mean$\pm$Stdev, with the maximum in parentheses below. MRPC and QQP scores are averaged for brevity. For experiments with the full training set, we omit tasks with more than 10k training examples, as BERT fine-tuning is generally more stable with sufficient data.}
\label{tab:glueresults_std}
\end{table*}


\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrrr@{/}rr@{/}rr@{/}rrrrr}
\toprule
% && \multicolumn{2}{c}{\textbf{Single Sentence}} & \multicolumn{3}{c}{\textbf{Similarity and Paraphrase}} & \multicolumn{4}{c}{\textbf{Natural Language Inference}} \\
\textbf{} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{1}{c}{\textbf{AvgEx}} & \multicolumn{1}{c}{\textbf{CoLA}} & \multicolumn{1}{c}{\textbf{SST}} & \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{STS}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{QNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{WNLI}} \\
\textbf{Training Set Size}&&&\multicolumn{1}{c}{\textit{8.5k}} & \multicolumn{1}{c}{\textit{67k}} & \multicolumn{2}{c}{\textit{3.7k}} & \multicolumn{2}{c}{\textit{364k}} & \multicolumn{2}{c}{\textit{7k}} & \multicolumn{1}{c}{\textit{393k}} & \multicolumn{1}{c}{\textit{108k}} & \multicolumn{1}{c}{\textit{2.5k}} & \multicolumn{1}{c}{\textit{634}}\\
\midrule
\midrule
\multicolumn{15}{c}{Development Set Scores} \\
\midrule
\textbf{LM} & 75.4 & 72.4 & \textbf{50.2} & \textbf{93.2} & 80.1 & 85.9 & 89.4 & 85.9 & 86.4 & 86.5 & \textbf{81.2} & 82.4 & 58.1 & 56.3 \\
\textbf{LM$\rightarrow$QQP} & 76.0 & 73.1 & 48.3 & 93.1 & 83.1 & 88.0 & *89.4 & 85.9 & 87.0 & 86.9 & 80.7 & 82.6 & 62.8 & 56.3 \\
\textbf{LM$\rightarrow$MNLI} & 76.7 & 74.2 & 45.7 & 92.2 & \textbf{87.3} & \textbf{90.8} & 89.2 & 85.3 & 88.1 & 88.0 & *\textbf{81.2} & \textbf{82.6} & \textbf{67.9} & 56.3 \\
\textbf{LM$\rightarrow$SNLI} & 76.0 & 73.1 & 41.5 & 91.9 & 86.0 & 89.9 & 89.9 & 86.6 & \textbf{88.7} & \textbf{88.6} & 81.1 & 82.2 & 65.7 & 56.3 \\
\textbf{LM$\rightarrow$Real/Fake} & 76.6 & 73.9 & 49.5 & 91.4 & 83.6 & 88.6 & \textbf{90.1} & \textbf{86.9} & 87.9 & 87.8 & 81.0 & 82.5 & 66.1 & 56.3 \\
\midrule
\textbf{Overall Best} & \textbf{77.6} & \textbf{75.5} & \textbf{50.2} & \textbf{93.2} & \textbf{87.3} & \textbf{90.8} & \textbf{90.1} & \textbf{86.9} & \textbf{88.7} & \textbf{88.6} & \textbf{81.1} & \textbf{83.1} & \textbf{67.9} & \textbf{56.3} \\
\midrule
\midrule
\multicolumn{15}{c}{Test Set Scores} \\
\midrule
\textbf{LM} & 74.6 & 72.9 & 47.2 & \textbf{93.1} & 84.7 & 79.1 & 87.7 & 69.3 & 81.5 & 79.6 & 80.7 & 86.6 & 57.8 & 65.1 \\
\textbf{LM$\rightarrow$QQP} & 75.4 & 74.1 & 45.5 & 92.6 & 79.8 & 85.2 & *87.7 & 69.3 & 84.0 & 82.7 & 80.1 & 86.9 & 64.0 & 65.1 \\
\textbf{LM$\rightarrow$MNLI} & 76.5 & 75.3 & 43.8 & 93.0 & 87.7 & 83.7 & 88.4 & 70.0 & 84.7 & 83.9 & *80.7 & \textbf{87.2} & \textbf{69.1} & 65.1 \\
\textbf{LM$\rightarrow$SNLI} & 75.7 & 74.3 & 39.4 & 91.0 & \textbf{84.1} & \textbf{88.2} & \textbf{88.2} & \textbf{70.3}  & \textbf{85.3} & \textbf{84.8} & 80.5 & 86.6 & 67.8 & 65.1 \\
\textbf{LM$\rightarrow$Real/Fake} & 76.2 & 75.0 & \textbf{47.9} & 92.8 & 82.8 & 87.6 & 88.1 & 70.1 & 84.0 & 82.7 & \textbf{80.8} & 86.4 & 65.5 & 65.1 \\
\midrule
%\textbf{Overall Best} & \textbf{77.0} & \textbf{78.0} & \textbf{47.9} & \textbf{93.1} & \textbf{84.1} & \textbf{88.2} & \textbf{88.2} & \textbf{70.3 & 85.3 & 84.8 & 80.8 & 79.6 & 69.1 & 65.1  \\
\textbf{Best based on Dev} & \textbf{76.9} & \textbf{75.9} & 47.2 & \textbf{93.1} & 87.7 & 83.7 & 88.1 & 70.1 & \textbf{85.3} & \textbf{84.8} & 80.7 & \textbf{87.2} & \textbf{69.1} & 65.1 \\
\bottomrule
\end{tabular}
\caption{GLUE results with and without STILTs, fine-tuning on full training data of each target task \underline{with} an auxiliary language modeling objective. \textbf{Bold} the best within each section. *~indicates cases where the intermediate task is the same as the target task--we substitute the baseline result for that cell. \textit{AvgEx} is the average excluding MNLI and QQP because of the overlap with intermediate tasks. See text for discussion of WNLI results.}
\label{tab:glueresults_old}
\end{table*}


\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrrr@{/}rr@{/}rr@{/}rrrrr}
\toprule
% && \multicolumn{2}{c}{\textbf{Single Sentence}} & \multicolumn{3}{c}{\textbf{Similarity and Paraphrase}} & \multicolumn{4}{c}{\textbf{Natural Language Inference}} \\
\textbf{} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{1}{c}{\textbf{AvgEx}} & \multicolumn{1}{c}{\textbf{CoLA}} & \multicolumn{1}{c}{\textbf{SST}} & \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{STS}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{QNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{WNLI}} \\
\textbf{Training Set Size}&&&\multicolumn{1}{c}{\textit{8.5k}} & \multicolumn{1}{c}{\textit{67k}} & \multicolumn{2}{c}{\textit{3.7k}} & \multicolumn{2}{c}{\textit{364k}} & \multicolumn{2}{c}{\textit{7k}} & \multicolumn{1}{c}{\textit{393k}} & \multicolumn{1}{c}{\textit{108k}} & \multicolumn{1}{c}{\textit{2.5k}} & \multicolumn{1}{c}{\textit{634}}\\
\midrule
\midrule
\multicolumn{14}{c}{At Most 5k Training Examples for Target Tasks} \\
\midrule
\textbf{LM} & 71.5 & 70.9 & \textbf{50.2} & \textbf{91.1} & 80.1 & 85.9 & 80.6 & 75.2 & 86.1 & 85.9 & 68.5 & 72.8 & 58.1 & 56.3 \\
\textbf{LM$\rightarrow$QQP} & 70.9 & 70.4 & 40.4 & 89.7 & 83.1 & 88.0 & *80.6&75.2 & 86.9 & 86.7 & 67.4 & 72.6 & 62.8 & 56.3 \\
\textbf{LM$\rightarrow$MNLI} & 73.0 & 72.4 & 44.2 & 88.9 & \textbf{87.3} & \textbf{90.8} & \textbf{82.2} & \textbf{77.1} & 87.3 & 87.2 & *68.8 & 74.8 & \textbf{67.9} & 56.3 \\
\textbf{LM$\rightarrow$SNLI} & 72.7 & 70.5 & 33.1 & 89.7 & 86.0 & 89.9 & 81.9 & 76.4 & \textbf{88.4} & \textbf{88.3} & \textbf{79.1} & \textbf{75.3} & 65.7 & 56.3 \\
\textbf{LM$\rightarrow$Real/Fake} & 73.8 & 72.2 & 48.3 & 89.7 & 83.6 & 88.6 & 81.5 & 76.3 & 87.3 & 87.1 & 78.0 & 73.4 & 66.1 & 56.3 \\
\midrule
\textbf{Overall Best} & \textbf{76.3} & \textbf{74.0} & \textbf{50.2} & \textbf{91.1} & \textbf{87.3} & \textbf{90.8} & \textbf{82.2} & \textbf{77.1} & \textbf{88.4} & \textbf{88.3} & \textbf{79.1} & \textbf{75.3} & \textbf{67.9} & \textbf{56.3} \\
\midrule
\midrule
\multicolumn{14}{c}{At Most 1k Training Examples for Target Tasks} \\
\midrule
\textbf{LM} & 58.3 & 60.2 & 0.0 & \textbf{88.4} & 73.3 & 82.8 & 73.0 & 66.7 & 81.0 & 80.6 & 35.0 & 63.0 & 53.1 & 56.3 \\
\textbf{LM$\rightarrow$QQP} & 63.8 & 63.0 & 12.1 & 85.8 & 73.8 & 82.0 & *73.0&66.7 & 79.5 & 79.9 & 60.4 & 69.1 & 61.7 & 56.3 \\
\textbf{LM$\rightarrow$MNLI} & 62.8 & 64.6 & 9.4 & 86.5 & 78.9 & 85.2 & \textbf{78.0} & \textbf{71.6} & 83.5 & 83.5 & *35.0 & \textbf{71.7} & \textbf{66.1} & 56.3 \\
\textbf{LM$\rightarrow$SNLI} & 67.7 & 65.0 & 11.7 & 86.1 & \textbf{83.6} & \textbf{88.5} & 77.8 & 69.9 & \textbf{85.1} & \textbf{85.1} & 77.5 & 69.5 & 63.2 & 56.3 \\
\textbf{LM$\rightarrow$Real/Fake} & 70.4 & 68.7 & \textbf{40.9} & 86.8 & 77.5 & 84.8 & 77.2 & 69.7 & 81.6 & 81.6 & \textbf{77.8} & 70.0 & 65.7 & 56.3 \\
\midrule
\textbf{Overall Best} & \textbf{73.7} & \textbf{70.7} & \textbf{40.9} & \textbf{88.4} & \textbf{83.6} & \textbf{88.5} & \textbf{78.0} & \textbf{71.6}  & \textbf{85.1} & \textbf{85.1} & \textbf{77.8} & \textbf{71.7} & \textbf{66.1} & 56.3 \\
\bottomrule
\end{tabular}
\caption{GLUE results on development set based on fine-tuning on only a subset of target-task data, simulating data-constrained scenarios, \underline{with} an auxiliary language modeling objective. \textbf{Bold} indicates the best within each section. *~indicates cases where the intermediate task is the same as the target task: We substitute the baseline result for that cell. \textit{AvgEx} is the average excluding MNLI and QQP because of the overlap with intermediate tasks. See text for discussion of WNLI results.}
\label{tab:glueresults_small_old}
\end{table*}


\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrrr@{/}rr@{/}rr@{/}rrrrr}
\toprule
% && \multicolumn{2}{c}{\textbf{Single Sentence}} & \multicolumn{3}{c}{\textbf{Similarity and Paraphrase}} & \multicolumn{4}{c}{\textbf{Natural Language Inference}} \\
\textbf{} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{1}{c}{\textbf{AvgEx}} & \multicolumn{1}{c}{\textbf{CoLA}} & \multicolumn{1}{c}{\textbf{SST}} & \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{STS}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{QNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{WNLI}} \\
\textbf{Training Set Size}&&&\multicolumn{1}{c}{\textit{8.5k}} & \multicolumn{1}{c}{\textit{67k}} & \multicolumn{2}{c}{\textit{3.7k}} & \multicolumn{2}{c}{\textit{364k}} & \multicolumn{2}{c}{\textit{7k}} & \multicolumn{1}{c}{\textit{393k}} & \multicolumn{1}{c}{\textit{108k}} & \multicolumn{1}{c}{\textit{2.5k}} & \multicolumn{1}{c}{\textit{634}}\\
\midrule
\midrule
\textbf{LM} & 75.3 & 72.7 & \textbf{52.8} & \textbf{92.3} & 80.6 & 86.4 & 88.2 & 84.6 & 87.5 & 87.2 & 79.6 & 81.5 & 57.8 & 56.3 \\
\textbf{LM$\rightarrow$QQP} & 73.1 & 69.7 & 29.8 & 91.4 & 82.8 & 87.7 & *88.2 & 84.6 & 87.4 & 87.3 & 80.1 & 78.9 & 62.8 & 56.3 \\
\textbf{LM$\rightarrow$MNLI} & 76.2 & 74.1 & 41.5 & 91.9 & \textbf{86.8} & \textbf{90.8} & 88.8 & 81.3 & 89.2 & 89.0 & *79.6 & \textbf{83.1} & \textbf{70.4} & 56.3 \\
\textbf{LM$\rightarrow$SNLI} & 75.4 & 72.5 & 35.3 & 90.9 & 86.3 & 90.2 & \textbf{89.0} & \textbf{85.4} & \textbf{90.1} & \textbf{89.8} & \textbf{81.2} & 82.9 & 66.4 & 56.3 \\
\textbf{LM$\rightarrow$Real/Fake} & 74.9 & 71.9 & 50.3 & 92.1 & 78.2 & 85.2 & 88.4 & 84.7 & 88.3 & 88.1 & \textbf{81.2} & 81.8 & 56.3 & 56.3 \\
\midrule
\textbf{Overall Best} & \textbf{78.0} & \textbf{75.9} & \textbf{52.8} & \textbf{92.3} & \textbf{86.8} & \textbf{90.8} & \textbf{89.0} & \textbf{85.4} & \textbf{90.1} & \textbf{89.8} & \textbf{81.2} & \textbf{83.1} & \textbf{70.4} & 56.3 \\
\bottomrule
\end{tabular}
\caption{Results on the GLUE development set with and without STILTs, fine-tuning on full training data of each target task, \underline{without} an auxiliary language modeling objective. \textbf{Bold} indicates the best within each section. *~indicates cases where the intermediate task is the same as the target task--we substitute the baseline result for that cell. \textit{AvgEx} is the average excluding MNLI and QQP because of the overlap with intermediate tasks. See text for discussion of WNLI results. 
}
\label{tab:glueresults_nolm}
\end{table*}


\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrrr@{/}rr@{/}rr@{/}rrrrr}
\toprule
% && \multicolumn{2}{c}{\textbf{Single Sentence}} & \multicolumn{3}{c}{\textbf{Similarity and Paraphrase}} & \multicolumn{4}{c}{\textbf{Natural Language Inference}} \\
\textbf{} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{1}{c}{\textbf{AvgEx}} & \multicolumn{1}{c}{\textbf{CoLA}} & \multicolumn{1}{c}{\textbf{SST}} & \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{STS}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{QNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{WNLI}} \\
\textbf{Training Set Size}&&&\multicolumn{1}{c}{\textit{8.5k}} & \multicolumn{1}{c}{\textit{67k}} & \multicolumn{2}{c}{\textit{3.7k}} & \multicolumn{2}{c}{\textit{364k}} & \multicolumn{2}{c}{\textit{7k}} & \multicolumn{1}{c}{\textit{393k}} & \multicolumn{1}{c}{\textit{108k}} & \multicolumn{1}{c}{\textit{2.5k}} & \multicolumn{1}{c}{\textit{634}}\\
\midrule
\midrule
\multicolumn{14}{c}{At Most 5k Training Examples for Target Tasks} \\
\midrule
\textbf{LM} & 71.6 & 71.2 & \textbf{50.8} & \textbf{91.1} & 81.4 & 87.1 & 79.5 & 73.8 & 87.6 & 87.4 & 68.8 & 73.1 & 56.3 & 56.3 \\
\textbf{LM$\rightarrow$QQP} & 65.2 & 63.3 & 0.0 & 82.0 & 82.8 & 87.7 & *79.5 & 73.8 & 87.4 & 87.3 & 65.1 & 71.6 & 62.8 & 56.3 \\
\textbf{LM$\rightarrow$MNLI} & 72.3 & 71.8 & 35.3 & 89.4 & \textbf{86.8} & \textbf{90.8} & \textbf{81.6} & \textbf{76.3} & 88.8 & 88.7 & *68.8 & 74.1 & \textbf{70.4} & 56.3 \\
\textbf{LM$\rightarrow$SNLI} & 72.3 & 70.2 & 29.6 & 89.2 & 86.3 & 90.2 & 81.6 & 76.0 & 89.5 & 89.4 & \textbf{78.3} & \textbf{74.7} & 66.4 & 56.3 \\
\textbf{LM$\rightarrow$Real/Fake} & 71.4 & 69.3 & 45.1 & 87.8 & 78.2 & 85.2 & 80.6 & 75.4 & \textbf{87.8} & \textbf{87.5} & 77.5 & 72.2 & 56.3 & 56.3 \\
\midrule
\textbf{Overall Best} & \textbf{75.4} & \textbf{74.3} & \textbf{50.8} & \textbf{91.1} & \textbf{86.8} & \textbf{90.8} & \textbf{81.6} & \textbf{76.3} & \textbf{89.5} & \textbf{89.4} & \textbf{78.3} & \textbf{74.7} & \textbf{70.4} & 56.3 \\
\midrule
\midrule
\multicolumn{14}{c}{At Most 1k Training Examples for Target Tasks} \\
\midrule
\textbf{LM} & 64.5 & 64.8 & 33.4 & 85.3 & 70.1 & 81.3 & 75.3 & 67.7 & 80.8 & 80.8 & 55.7 & 66.7 & 54.9 & 56.3 \\
\textbf{LM$\rightarrow$QQP} & 64.6 & 64.6 & 23.0 & \textbf{87.0} & 74.8 & 83.2 & *75.3 & 67.7 & 84.4 & 84.3 & 57.8 & 67.1 & 55.2 & 56.3 \\
\textbf{LM$\rightarrow$MNLI} & 65.2 & 65.2 & 13.3 & 86.2 & 79.2 & 85.8 & \textbf{78.4} & \textbf{70.5} & 86.2 & 86.1 & *55.7 & 68.6 & \textbf{63.2} & 56.3 \\
\textbf{LM$\rightarrow$SNLI} & 67.5 & 64.9 & 13.4 & 85.7 & \textbf{80.1} & \textbf{86.2} & 77.2 & 70.0 & \textbf{87.5} & \textbf{87.5} & \textbf{76.8} & \textbf{70.3} & 60.6 & 56.3 \\
\textbf{LM$\rightarrow$Real/Fake} & 65.3 & 62.5 & \textbf{36.3} & 69.7 & 69.6 & 79.6 & 75.5 & 69.4 & 84.7 & 84.8 & 74.6 & 69.1 & 50.2 & 56.3 \\
\midrule
\textbf{Overall Best} & \textbf{70.6} & \textbf{68.9} & \textbf{36.3} & \textbf{87.0} & \textbf{80.1} & \textbf{86.2} & \textbf{78.4} & \textbf{70.5} & \textbf{87.5} & \textbf{87.5} & \textbf{76.8} & \textbf{70.3} & \textbf{63.2} & 56.3 \\
\bottomrule
\end{tabular}
\caption{Results on the GLUE development set based on fine-tuning on only a subset of target-task data, simulating data scarce scenarios, \underline{without} an auxiliary language modeling objective. \textbf{Bold} indicates the best within each section. *~indicates cases where the intermediate task is the same as the target task: We substitute the baseline result for that cell. \textit{AvgEx} is the average excluding MNLI and QQP because of the overlap with intermediate tasks. See text for discussion of WNLI results.}
\label{tab:glueresults_nolm_small}
\end{table*}








% BERT 1k/5k Old
\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrrrrrrrrc}
\toprule
% && \multicolumn{2}{c}{\textbf{Single Sentence}} & \multicolumn{3}{c}{\textbf{Similarity and Paraphrase}} & \multicolumn{4}{c}{\textbf{Natural Language Inference}} \\
\textbf{} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{1}{c}{\textbf{AvgEx}} & \multicolumn{1}{c}{\textbf{CoLA}} & \multicolumn{1}{c}{\textbf{SST}} & \multicolumn{1}{c}{\textbf{MRPC}} & \multicolumn{1}{c}{\textbf{QQP}} & \multicolumn{1}{c}{\textbf{STS}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{QNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{WNLI}} \\
\textbf{Training Set Size}&&&\multicolumn{1}{c}{\textit{8.5k}} & \multicolumn{1}{c}{\textit{67k}} & \multicolumn{1}{c}{\textit{3.7k}} & \multicolumn{1}{c}{\textit{364k}} & \multicolumn{1}{c}{\textit{7k}} & \multicolumn{1}{c}{\textit{393k}} & \multicolumn{1}{c}{\textit{108k}} & \multicolumn{1}{c}{\textit{2.5k}} & \multicolumn{1}{c}{\textit{634}}\\
\midrule
\midrule
\multicolumn{11}{c}{At Most 5k Training Examples for Target Tasks} \\
\midrule
\textbf{BERT}& 79.2 & 79.3 & 60.6 & 93.5 & 89.1 & 90.0 & 80.9 & 77.1 & 82.8 & 74.0 & 65.1 \\
&&& (27.2) & (18.1) & (6.6) & (21.1) & (21.1) & (20.9) & (11.5) & (8.2) & -  \\
\textbf{BERT$\rightarrow$QQP}& 79.5 & 78.7 & 55.3 & 92.0 & 89.7 & 90.6 & 88.9 & 75.9 & 81.6 & 76.5 & 65.1 \\
&&& (23.3) & (0.9) & (5.6) & (32.4) & (0.2) & (15.1) & (12.3) & (9.1) & -  \\
\textbf{BERT$\rightarrow$MNLI} & 81.4 & 80.9 & 59.6 & 92.4 & 91.0 & 90.9 & 80.9 & 85.6 & 83.9 & 83.4 & 65.1 \\
&&& (16.7) & (9.1) & (1.1) & (22.1) & (17.9) & (0.3) & (10.1) & (6.3) & -  \\
\textbf{BERT$\rightarrow$SNLI} & 79.8 & 79.6 & 56.6 & 91.5 & 89.9 & 90.7 & 80.4 & 80.6 & 82.7 & 80.5 & 65.1 \\
&&& (22.4) & (1.0) & (5.0) & (20.8) & (22.6) & (10.8) & (11.7) & (11.2) & -  \\
\textbf{BERT$\rightarrow$Real/Fake} & 72.0 & 72.9 & 53.6 & 88.9 & 85.1 & 88.4 & 78.9 & 59.1 & 74.1 & 54.9 & 65.1 \\
&&& (22.9) & (17.0) & (3.3) & (40.6) & (18.0) & (7.1) & (8.3) & (2.0) & -  \\
\midrule
\textbf{Overall Best} & . & . & . & . & . & . & . & . & . & . & . \\
\midrule
\midrule
\multicolumn{11}{c}{At Most 1k Training Examples for Target Tasks} \\
\midrule
\textbf{BERT} & 75.2 & 75.7 & 54.0 & 91.1 & 86.1 & 88.0 & 76.8 & 69.7 & 77.0 & 69.0 & 65.0 \\
&&& (17.5) & (17.9) & (3.7) & (20.2) & (17.4) & (13.7) & (9.9) & (7.2) & -  \\
\textbf{BERT$\rightarrow$QQP} & 75.5 & 74.7 & 47.5 & 89.7 & 84.5 & 88.5 & 88.6 & 67.5 & 76.4 & 71.5 & 65.0 \\
&&& (16.6) & (11.4) & (2.1) & (13.8) & (0.4) & (13.1) & (2.2) & (8.3) & -  \\
\textbf{BERT$\rightarrow$MNLI} & 77.8 & 76.8 & 44.0 & 90.5 & 87.8 & 88.7 & 77.3 & 84.9 & 79.0 & 82.7 & 65.0 \\
&&& (16.5) & (8.6) & (1.6) & (0.7) & (13.8) & (0.4) & (6.3) & (1.5) & -  \\
\textbf{BERT$\rightarrow$SNLI} & 76.4 & 76.0 & 47.6 & 89.3 & 85.3 & 88.0 & 77.4 & 78.6 & 77.6 & 79.1 & 65.0 \\
&&& (20.2) & (14.8) & (3.2) & (1.1) & (16.2) & (10.9) & (9.6) & (7.1) & -  \\
\textbf{BERT$\rightarrow$Real/Fake} & 64.9 & 68.2 & 43.9 & 72.5 & 81.8 & 82.8 & 71.2 & 35.3 & 69.7 & 61.7 & 65.0 \\
&&& (18.0) & (5.2) & (1.9) & (22.7) & (16.9) & (1.2) & (4.4) & (3.7) & -  \\
\midrule
\textbf{Overall Best} & . & . & . & . & . & . & . & . & . & . & . \\
\bottomrule
\end{tabular}
\caption{GLUE results on development set based on fine-tuning on only a subset of target-task data, simulating data-constrained scenarios, \underline{with} an auxiliary language modeling objective. \textbf{Bold} indicates the best within each section. *~indicates cases where the intermediate task is the same as the target task: We substitute the baseline result for that cell. \textit{AvgEx} is the average excluding MNLI and QQP because of the overlap with intermediate tasks. See text for discussion of WNLI results.}
\label{tab:glueresults_small_old}
\end{table*}


\begin{table*}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrrrrrrrrc}
\toprule
% && \multicolumn{2}{c}{\textbf{Single Sentence}} & \multicolumn{3}{c}{\textbf{Similarity and Paraphrase}} & \multicolumn{4}{c}{\textbf{Natural Language Inference}} \\
\textbf{} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{1}{c}{\textbf{AvgEx}} & \multicolumn{1}{c}{\textbf{CoLA}} & \multicolumn{1}{c}{\textbf{SST}} & \multicolumn{1}{c}{\textbf{MRPC}} & \multicolumn{1}{c}{\textbf{QQP}} & \multicolumn{1}{c}{\textbf{STS}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{QNLI}} & \multicolumn{1}{c}{\textbf{RTE}}  \\
\textbf{xx}&&&\multicolumn{1}{c}{\textit{8.5k}} & \multicolumn{1}{c}{\textit{67k}} & \multicolumn{1}{c}{\textit{3.7k}} & \multicolumn{1}{c}{\textit{364k}} & \multicolumn{1}{c}{\textit{7k}} & \multicolumn{1}{c}{\textit{393k}} & \multicolumn{1}{c}{\textit{108k}} & \multicolumn{1}{c}{\textit{2.5k}} \\
\midrule
\midrule
\multicolumn{11}{c}{At Most 5k Training Examples for Target Tasks} \\
\midrule
\textbf{BERT}& 79.2 & 79.3 & 60.6 & 93.5 & 89.1 & 90.0 & 80.9 & 77.1 & 82.8 & 74.0 & 65.1 \\
&&& (27.2) & (18.1) & (6.6) & (21.1) & (21.1) & (20.9) & (11.5) & (8.2) & -  \\
\textbf{$\rightarrow$QQP}& 79.5 & 78.7 & 55.3/70.0 & 92.0/70.0 & 89.7/70.0 & 90.6/70.0 & 88.9/70.0 & 75.9/70.0 & 81.6/70.0 & 76.5/70.0 & 65.1/70.0 \\
&&& (23.3) & (0.9) & (5.6) & (32.4) & (0.2) & (15.1) & (12.3) & (9.1) & -  \\
\textbf{$\rightarrow$MNLI} & 81.4 & 80.9 & 59.6 & 92.4 & 91.0 & 90.9 & 80.9 & 85.6 & 83.9 & 83.4 & 65.1 \\
&&& (16.7) & (9.1) & (1.1) & (22.1) & (17.9) & (0.3) & (10.1) & (6.3) & -  \\
\textbf{$\rightarrow$SNLI} & 79.8 & 79.6 & 56.6 & 91.5 & 89.9 & 90.7 & 80.4 & 80.6 & 82.7 & 80.5 & 65.1 \\
&&& (22.4) & (1.0) & (5.0) & (20.8) & (22.6) & (10.8) & (11.7) & (11.2) & -  \\
\textbf{$\rightarrow$Real/Fake} & 72.0 & 72.9 & 53.6 & 88.9 & 85.1 & 88.4 & 78.9 & 59.1 & 74.1 & 54.9 & 65.1 \\
&&& (22.9) & (17.0) & (3.3) & (40.6) & (18.0) & (7.1) & (8.3) & (2.0) & -  \\
\midrule
\textbf{Overall Best} & . & . & . & . & . & . & . & . & . & . & . \\
\midrule
\midrule
\multicolumn{11}{c}{At Most 1k Training Examples for Target Tasks} \\
\midrule
\textbf{BERT} & 75.2 & 75.7 & 54.0 & 91.1 & 86.1 & 88.0 & 76.8 & 69.7 & 77.0 & 69.0 & 65.0 \\
&&& (17.5) & (17.9) & (3.7) & (20.2) & (17.4) & (13.7) & (9.9) & (7.2) & -  \\
\textbf{$\rightarrow$QQP} & 75.5 & 74.7 & 47.5 & 89.7 & 84.5 & 88.5 & 88.6 & 67.5 & 76.4 & 71.5 & 65.0 \\
&&& (16.6) & (11.4) & (2.1) & (13.8) & (0.4) & (13.1) & (2.2) & (8.3) & -  \\
\textbf{$\rightarrow$MNLI} & 77.8 & 76.8 & 44.0 & 90.5 & 87.8 & 88.7 & 77.3 & 84.9 & 79.0 & 82.7 & 65.0 \\
&&& (16.5) & (8.6) & (1.6) & (0.7) & (13.8) & (0.4) & (6.3) & (1.5) & -  \\
\textbf{$\rightarrow$SNLI} & 76.4 & 76.0 & 47.6 & 89.3 & 85.3 & 88.0 & 77.4 & 78.6 & 77.6 & 79.1 & 65.0 \\
&&& (20.2) & (14.8) & (3.2) & (1.1) & (16.2) & (10.9) & (9.6) & (7.1) & -  \\
\textbf{$\rightarrow$Real/Fake} & 64.9 & 68.2 & 43.9 & 72.5 & 81.8 & 82.8 & 71.2 & 35.3 & 69.7 & 61.7 & 65.0 \\
&&& (18.0) & (5.2) & (1.9) & (22.7) & (16.9) & (1.2) & (4.4) & (3.7) & -  \\
\midrule
\textbf{Overall Best} & . & . & . & . & . & . & . & . & . & . & . \\
\bottomrule
\end{tabular}
\caption{GLUE results on development set based on fine-tuning on only a subset of target-task data, simulating data-constrained scenarios, \underline{with} an auxiliary language modeling objective. \textbf{Bold} indicates the best within each section. *~indicates cases where the intermediate task is the same as the target task: We substitute the baseline result for that cell. \textit{AvgEx} is the average excluding MNLI and QQP because of the overlap with intermediate tasks. See text for discussion of WNLI results.}
\label{tab:glueresults_small_old}
\end{table*}


\begin{table}[t]
\centering \small \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lrrrr}
\toprule
\textbf{Setup} & \textbf{GPT} & \textbf{STILTs} & \textbf{MTL1} &\textbf{MTL2}\\
\midrule
\textbf{RTE Accuracy} & 54.2 & \textbf{70.4} & 68.6 & 67.5\\
\bottomrule
\end{tabular}
\caption{Comparison of STILTs against multi-task learning setups for GPT without the auxiliary language model loss on the RTE target task with MNLI as an auxiliary task}
\label{tab:mtexp}
\end{table}
